The Impact of Incomplete Information on Network Formation with Heterogeneous Agents

We propose an agent-based network formation model under uncertainty with the objective of relaxing the common assumption of complete information, calling attention to the role beliefs may play in segregation. We demonstrate that our model is capable of generating a set of networks that encompasses those of a complete information model. Further, we show that by allowing agents to be biased toward each other based on observable attributes, our model is able to generate homophilous equilibria with preferences that are indifferent to these attributes. We accompany our theoretical results with a simulation-based investigation of the relationship between beliefs and segregation and show that biased beliefs are an important driver of segregation under incomplete information.

==> cover.tex <==
As per our application through the fast track, in this cover letter we provide the reviews (and post rebuttal comments) that we received when submitting to AAMAS-2021.

Review 1
Summary:	This paper shows, both in theoretical terms as well as experimental terms (with simulation), the role that observable traits and unobservable traits have in the phenomenon called homophily. The idea that information is incomplete (with respect to who you do not know) provides another explanation for homophily than that homophily was simply an assumed preference itself.
Strengths:	This is a very clear language, compact paper. The first half describes the reasoning mathematically. The second half provides simulation outcomes and does so clearly and convincingly. The paper is very complete until presenting those outcomes.
Weaknesses:	The modelling is somewhat limited in scope: it only simulates with 12 agents and differentiates only two unobservable states. This may be sufficient for understanding the general patterns, but it is not clear whether other patterns would emerge under different starting positions (unevenly sized social groups, for instance).
Detailed comments:	Scores good on all criteria mentioned. It simply is a convincing paper, well focused on studying a possible source for homophily to emerge when networks form.
Questions for rebuttal:	
Score:	
5: (borderline (but tending towards rejection))
Comments added after rebuttal:	I like the model introduced in the paper but, but the model results are limited. I have had only little reference to earlier AAMAS papers for determining the overall judgement; the discussion and have helped me to come to a more appropriate overall judgement in view of the scoring practices for AAMAS.


Review 2
Summary:	The paper studies a network creation game with heterogeneous agents and incomplete information. The model is an extension of the well-known model of network formation introduced by Jackson and Wolinsky in [16] in which players are nodes of a network that has to be built.

In this new model, there are N agents that are grouped into K social groups. Each agent belongs to a single group and the groups are common knowledge. Moreover, each agent i has also a type t_i. t_i is private and at the beginning it is known only by agent i and then it is discovered by any agent j that meets agent i during the network formation process (two agents i and j meet whenever they agree to form link ij).

Given a state of the game, namely the set of formed links and thus a graph g, a player i has an \emph{actual} utility/payoff in g defined by Equation (1). In Eq. (1), the cost term is the sum of the costs of the links incident to i, and the cost of a specific link ij depends on t_i and t_j.
So far the model is the same as Jackson and Wolinsky's one.
Here comes the novelty: when player i evaluates the possibility of forming a new link ij (not belonging to the actual graph g), it might happen that i and j have never met. In this case, agent i does not know j's type t_j and cannot evaluate the actual utility in g+ij. Instead, it computes an expected utility in g+ij in which the cost of forming link ij is the average of the costs to connect with each type t weighted by agent i's belief that agent j is of type t given their social group. i and j thus forms link ij only if their expected utilities are non-negative, they thus meet each other and discover their actual types.

The authors provide the following results:

(1) They prove some formal propositions about the set of equilibria of the game. They use pairwise stability as solution concept. For example, they derive some conditions under which the complete graph is an equilibrium or in which the empty network is not. They also argue that the set of stable networks in the complete information version of the game is strictly included into the one of stable networks for the incomplete information counterpart.

(2) They run some experiments by simulating the dynamic network formation process in order to understand how segregation and connectivity indices vary as different parameters of the model vary. Their main aim is to investigate the role of uncertainty (and hence the role of the specific belief mechanism) in the game.
Strengths:	I think that the model of network formation game introduced in the paper is really nice. In particular, I liked a lot the fact that the model manages the incomplete information about the types of the other unknown agents by introducing the notion of beliefs. This is vaguely inspired by the field of psychology and it allows for a particularly nice kind of heterogeneous agents.
Weaknesses:	My feeling is that both results (1) and (2) are weak from a technical point of view. Results of (1) are simple properties that directly follows from the definition of the model and can be proved by using quite trivial calculations.
Concerning (2), it seems to me that the outcomes of the experiments are somewhat expected, like for instance the fact that the degree of segregation increases as the inter-type cost (C_H) increases. Moreover, the authors consider only networks with 12 nodes (and 2 groups and 2 types). I have some doubt about the fact that simulations over 12-node networks could provide deep insights about real social networks.
Detailed comments:	Minor comments:

- In Equation (3) please explicitly say that distances d_{ik} are defined according to the network g+ij.

- Proof of Proposition 1. Page 3, column 1, last line. It seems to me that "E[u_{ij}]=\delta -..." should be "E[u_{ij}] \ge \delta -..." since agent i could get more benefit from agents that get closer to i via link ij.

- Equation (10). Please say (ore repeat if it is defined somewhere else) that n_k is the cardinality of group k.
Questions for rebuttal:	
Score:	
4: (poor (good attempt but too many concerns, so probably should be rejected))
Comments added after rebuttal:	Thanks for the further explanations. As I already said, I really like the model introduced in the paper. However, I still have doubts about the significance of the results. The paper is good but maybe a bit below the standard of AAMAS.


Review 3
Summary:	This paper proposes a network formation model where agents seek to connect with other agents of the same type in an environment where agents have incomplete information about the types of the other agents. In place of information about the types, agents have knowledge of some observable characteristics (called a “social group”) of each other agent that may or may not be correlated with the underlying type. It is noteworthy that this model generalizes network formation models with complete information.

The introduction of the distinction between hidden types and observable groups allows for the exploration of the effect of biased beliefs, where an agent (erroneously) believes a member of their social group is more likely to share their underlying type. When agents have biased beliefs, homophilous equilibria (with respect to groups) are shown to be able to emerge, even though agents only have homophilous preferences with respect to type.
Strengths:	Applying beliefs and uncertainty to network formation is an interesting way to extend previous work. The model proposed in the paper is well-motivated and a natural extension of network formation models under complete information. Further, the generalized pairwise stability condition proves to be a useful solution concept for the theoretical results that nicely characterize the behavior of the system for various ranges of parameter values.
Weaknesses:	In general, the paper somewhat over-promises and under-delivers on the results. The assertion that the model generates homophilous outcomes despite non-homophilous obscures what really happens in the model. The proofs of the technical results are hard to follow due to missing details. The experimental results would benefit from considering a few natural variations of the initial setup.
Detailed comments:	First, I think it is misleading to describe the results as generating homophilous outcomes without homophilous preferences, even given the distinction that the homophilous outcomes are with respect to social groups. Agents do have homophilous preferences: they prefer to connect to agents with the same hidden type. Types and groups are uncorrelated in the simulations, but biased agents believe that they are correlated, and that belief combined with their homophilous preferences for type is what drives the results.
This somewhat non-standard definition of homophily should be articulated more clearly in the statements of results and contributions. One way to help this would be differentiate it from the more standard notion of homophily by using a term like “social group homophily” or “homophily for observable characteristics.”

Second, the proofs of several of the theoretical results are opaque and hard to follow. There should be an appendix section or a full version of the paper (neither of which are mentioned) where the proofs are spelled out in greater detail, so that a reader may see the key ideas and verify the results without having to derive the proof on their own.
For example, the structure of the proofs of Proposition 1 and 2 is unclear. Both begin with the objective of a proof by contradiction, but it is not clear where the contradictions are derived later in the proofs.
The proof of Corollary 2 is even less clear. Proposition 2 gives sufficient conditions about when the empty network is unstable and Proposition 1 gives sufficient conditions about when agents i and j must know each other in a pairwise stable equilibrium, but (i) of Corollary 2 makes a claim about when the empty network must be stable, because no agents will have ever chosen to meet. Because Propositions 1 and 2 give sufficient conditions, but not also necessary conditions, (i.e. they are stated as “if” not “if and only if”) it is not at all clear how they imply this result in Corollary 2, and no details are given in the proof.

Third, for the simulations, there ought to be more discussion of the choice to keep types and groups independent. Ideally, there would be simulations for both cases.
Certainly, there are interesting cases in reality where it is plausible that the analogues of groups and types are independent, but it is by no means the only model or the natural model. There are similarly interesting cases where the analogues of groups and types would be correlated and those cases should similarly be explored
It would also be nice to have the agents update their beliefs over time as they meet other agents, as mentioned in the conclusion section.

Lastly, the paper is missing a key citation of Schelling’s widely-known work on agent based models related to segregation, which seems eminently relevant to this paper’s line of inquiry.

- Schelling, T.C. (1969). "Models of Segregation," American Economic Review (Papers and Proceedings), 59(2): 488-493.
- Schelling, T.C. (1971) "Dynamic models of segregation," The Journal of Mathematical Sociology, 1:143-186.
Questions for rebuttal:	
Score:	
4: (poor (good attempt but too many concerns, so probably should be rejected))
Comments added after rebuttal:	I just want to say that if you update it according to the rebuttal, it would make a nice AAMAS paper. Unfortunately, we need to judge based on the document submitted.

In particular, everyone really likes your model. It would be even better if slightly more could be done. Also, be cautious about over-selling your results.


Metareview for paper 160
Title: 	Uncertainty in Social Networks: The Impact of Incomplete Information on Network Formation with Heterogeneous Agents
Authors: 	D. Kai Zhang and Alexander Carver
Text: 	This paper shows a promising path of work that at this moment seems not to have delivered yet enough results to be accepted for AAMAS. I encourage the authors to continue, and hope the reviews help develop this research.



In response to these reviews, we have conducted the following changes.
- We have significantly increased the size of the simulations to 48 nodes to provide more confidence in our findings.
- We have simulated across a wider range of belief distributions and variations rather than relying on an arbitrary initial value.
- We have clarified both our proofs but also our wording relating to our claims to specify the importance of discovering emergent segregated, and non-optimal states for social welfare that would not occur without incomplete information and beliefs.
